Goal-Auxiliary Actor-Critic for 6D Robotic Grasping with Point Clouds

6D robotic grasping beyond top-down bin-picking scenarios is a challenging task. Previous solutions based on 6D grasp synthesis with robot motion planning usually operate in an open-loop setting, which are sensitive to grasp synthesis errors. In this work, we propose a new method for learning closed-loop control policies for 6D grasping. Our policy takes a segmented point cloud of an object from an egocentric camera as input, and outputs continuous 6D control actions of the robot gripper for grasping the object. We combine imitation learning and reinforcement learning and introduce a goal-auxiliary actor-critic algorithm for policy learning. We demonstrate that our learned policy can be integrated into a tabletop 6D grasping system and a human-robot handover system to improve the grasping performance of unseen objects. Our videos and code can be found at https://sites.google.com/view/gaddpg .

==> background.tex <==
 
\section{Background}
 
\label{sec:background}
 

\textbf{Markov Decision Process.} A Markov Decision Process (MDP) is defined using the tuple: $\mathcal{M}=\{\mathcal{S},\mathcal{R},\mathcal{A},\mathcal{O},\mathcal{P},\rho_0,\gamma \}$. $\mathcal{S}$, $\mathcal{A}$, and $\mathcal{O}$ represent the state, action, and observation space. $\mathcal{R}:\mathcal{S} \times \mathcal{A}\to \mathbb{R}$ is the reward function.   
$\mathcal{P}: \mathcal{S}\times \mathcal{A}\to \mathcal{S}$ is the transition dynamics. $\rho_0$ is the probability distribution over initial states and $\gamma=[0,1)$ is a discount factor. Let $\pi: \mathcal{S} \to \mathcal{A}$ be a policy which maps states to actions. In the partially observable case, at each time $t$, the
policy maps a partial observation $o_t$ of the environment to an action $a_t=\pi(o_t)$. Our goal is to learn a policy that maximizes the expected cumulative rewards $\EXP0_{\pi}[\sum_{t=0}^\infty \gamma^t r_t]$, where $r_t$ is the reward at time $t$. The Q-function of the policy for a state-action pair is $Q(s,a) =\mathcal{R}(s,a)+\gamma\EXP0_{s',  \pi}[\sum_{t=0}^\infty \gamma^tr_t|s_0=s']$, where $s'$ represents the next state of taking action $a$ in state $s$ according to the transition dynamics.


% \textbf{Imitation Learning.} Given a set of demonstration data in terms of state-action pairs from an expert $\mathcal{D}=\{(s,a)\}$, Behavior Clone (BC) can be applied on the states visited by the expert policy $ \pi^*$ to learn a policy $\pi_\theta$ via supervised learning. One problem with BC is the distribution shift: the state distribution over which the learner is trained is different from the  distribution of its own rollouts. This mismatch problem can be often corrected using DAGGER \cite{ross2011reduction}. In its simplest form, it augments $\mathcal{D}$ by adding expert supervision to the states visited by the learner policy $\pi_\theta$.

% Let $\theta$ parametrizes the learner policy $\pi$. Standard supervised learning is used to match the behavior of the expert with the maximum likelihood objective $ \max_{\theta} \EXP0_{(s,a) \sim \mathcal{D}}[ \ln(\pi_\theta(a|s))] $. 



\textbf{Deep Deterministic Policy Gradient.} DDPG \cite{lillicrap2015continuous} is an actor-critic algorithm that uses off-policy data, deterministic policy gradient, and temporal difference learning. It has successful applications in continuous control~ \cite{popov2017data,vecerik2017leveraging}. Specifically, the actor in DDPG learns the policy $\pi_{\theta}(s)$, while the critic approximates the Q-function $Q_{\phi}(s,a)$, where $\theta$ and $\phi$ denote the parameters of the actor and the critic, respectively. A replay buffer of transitions $\mathcal{D}=\{(s,a,r,s')\}$ is maintained during training, and examples sampled from it are used to optimize the actor and critic alternately. DDPG minimizes the following Bellman error with respect to $\phi$ :
\begin{equation}
  \EXP0_{(s,a,r,s')\sim \mathcal{D}} \Big[ \frac{1}{2}  \Big( Q_{\phi  }(s,a) - \big( r +\gamma  Q_{\phi  }(s',\pi_{\theta  }(s') \big) \Big) ^2 \Big].
\end{equation}
Then the deterministic policy $\pi_\theta$ is trained to maximize the learned Q-function with $\max_\theta \EXP0_{s\sim \mathcal{D}}(Q_\phi(s,\pi_\theta(s)))$, which resembles a policy evaluation and improvement schedule.

% To stabilize the training, multiple design choices are often used such as target networks, polyak averaging update, multiple Q networks, target policy smoothing, and delayed policy updates \cite{van2015deep,fujimoto2018addressing}.


%The deterministic policy gradient can be computed as  \begin{equation} 
%    \nabla_\theta {J}=\EXP0_{(s,a) \sim \mathcal{D}} \big[  \nabla_a Q_\phi(s,a)\nabla_\theta  \pi_\theta(s) \big].
%\end{equation} 

